Recommend for a Reason: Unlocking the Power of Unsupervised Aspect-Sentiment Co-Extraction

Compliments and concerns in reviews are valuable for understanding users' shopping interests and their opinions with respect to specific aspects of certain items. Existing review-based recommenders favor large and complex language encoders that can only learn latent and uninterpretable text representations. They lack explicit user attention and item property modeling, which however could provide valuable information beyond the ability to recommend items. Therefore, we propose a tightly coupled two-stage approach, including an Aspect-Sentiment Pair Extractor (ASPE) and an Attention-Property-aware Rating Estimator (APRE). Unsupervised ASPE mines Aspect-Sentiment pairs (AS-pairs) and APRE predicts ratings using AS-pairs as concrete aspect-level evidence. Extensive experiments on seven real-world Amazon Review Datasets demonstrate that ASPE can effectively extract AS-pairs which enable APRE to deliver superior accuracy over the leading baselines.

==> content/TODO.tex <==
Intro：
[x] 1. Change to review rating pred terminology
[D] 2. A sentence summarization of contribution!

Method:
[x] 1. whether to add table to discuss why three methods (each pros and cons) PMI, NN, Knowledge
[x] 2. intuition of dependency-based algorithm
[x] 3. add note to this section that appendix provides pseudo-code
[x] 4. PMI counting based, rather than lambda-based. (appendix, pseudocode)
[x] 5. rephrase about the `filtering`
[x] 6. now we are using $q$ as the quota
[x] 7. build sentiment term set -- change ``discrepancies'' to larger coverage
[x] 8. Add clamp to J($\Theta$)
[x] 9. Remove seeds from appendix
[x] 10. What converts sentiment to attention
[x] 11. Aspects not mentioned are zero

Experiments:
[x] 1. Add d-attn to the baselines
[x] 2. Solve the NeuMF 
[x] 4. Ablation studies (both are running, except DM - data damaged)
    [x] 4-0. Fix DM dataset
    [x] 4-1. Rerun ablation on DM
    [x] 4-2. Add ablation study in Sec-Experiment
    [x] 4-3. fill in the numbers in Table 6.
[x] 5. Two more datasets MSE (both are running working)
[x] 6. Two more datasets' statistics
[x] 7. Hyper-param sensitivity in Section-Exp
[x] 8. Hyper-param sensitivity in Section-App
[x] 9. Add ANH to Section App
[x] 10. Two more datasets' example 
[x] 11. Re-plot Figure 5.
[x] 13. Fill in Table 8: default parameter settings
[x] 14. Design and write case study.
[x] 15. remove lambda in appendix
[x] 16. Mention hugging face version
[x] 17. Add $d_a$ in experiments
[x] 18. mention run time in a separate section
[x] 19. Add dependency parser information spaCy
[x] 20. Add SDRN information
[x] 21. Separate #Trn/Rev # Tst/Rev in Table 2.
[x] 23. Add dot to ablation study figures
[x] 24. Mention in Case Study that it's joint for both ASPE and APRE
[x] 25. Mention Table8 is complicated
[x] 26. Table 5 caption, add asp/senti difference
[x] 27. Case study is actually all mentions, not example one or two
[x] 28. Add checkmarks and crosses to Table 5
[D] 29. Not a good option. Add efficiency to experiments
[x] 30. Fill in Table 4, the MSE
[x] 31. Run missing Experiments!
[x] 32. rephrase Ablation
[x] 33. Add another case study in Appendix
[x] 34. From to issue in Experiments (see chat box)
[x] 35. Add some colors to MSE table
[x] 36. Case study on "Sound"
[x] 37. Refine the ablation study figure!
[x] 38. Add cell color to two summarization tables
[x] 39. Fix all red sentences!
[x] 40. Fix all comments from Reema, including one sentence
[x] 41. Change data statistics table
[x] 42. Validation trails
[x] 43. Trn/Val/Test ratio 8:1:1
    [x] 43.1 Ratio in Paper
    [x] 43.2 Ratio in Data


[D] 22. Add to ablation study that ``pillow'' is true case.

Space limit
[x] 1. Table 2 to appendix. Remember to explain what are W/U/T/R in Table 2 caption.
[x] 2. Renamed ``supplimentary materials'' by \dagger sign.


MOST IMPORTANT!
[x] THINK ABOUT A GOOD TITLE!



Overall:
[x] 1. change knowledge to lexicon
[x] 2. write abstract
[x] 3. re-organized source code
    [x] 3-1. finish README.md in the source code
    [x] 3-2 remove less-related files from the source code
    [x] 3-3. Create anonymized copy of code
    [x] 3-4. Don't forget to submit a separate zip file of software.
[x] 5. Write broader Impact!!!
[x] 6. All attention to attentions!
[x] 7. dagger sign before and after space
[x] 8. Cite Bing Liu
[x] 9. Put in Paper ID (see WeChat)
[x] 10. Unify the format of references
[x] 11. Make sure all ref are correct!!!
[x] 12. All tables punctuation and caption.
[x] 13. Runtime table in Appendix
[x] 14. Grammarly the whole thing

==> tables/param_setting.tex <==
% \begin{table}[!ht]
%     \centering
%     \resizebox{\linewidth}{!}{
%     \begin{tabular}{ll|ll}
%         \topline
%         \rowcolor[gray]{.92}
%             Parameters & Values & Parameters & Values\\
%         \midtopline
%             BERT layers & 12 & & \\
%             BERT hidden & 768 & &\\
%             BERT head   & 12 & &\\
%             xx & & &\\
%         \bottomrule
%     \end{tabular}
%     }
%     \caption{Default hyper-parameters of our models. \td{change pattern}}
%     \label{tab:parameters}
% \end{table}


\begin{table}[!ht]
    \centering
        \resizebox{0.99\linewidth}{!}{%
    \begin{tabular}{rccccccc}
        \topline
        \rowcolor[gray]{.92}
        Hyper-params & \textsf{MI} & \textsf{AM} & \textsf{DM} & \textsf{PS} & \textsf{SO} & \textsf{TG} & \textsf{TH}  \\
        
        \midtopline
        \multicolumn{8}{c}{\small{\textsc{Settings for \tmn{} (AS-pair extraction)}}}\\
        
        Freq. threshold $c$ & & 50 & 100 & 150 & 250 & 150 & 150 \\
        Context size $w_\text{ctx}$& \multicolumn{7}{c}{5} \\
        % PMI min word freq. & \multicolumn{7}{c}{20} \\
        
        \midrule
        
        \multicolumn{8}{c}{\small{\textsc{Settings for \rmn{} (Rating prediction)}}}\\
        
        Review pad len. & \multicolumn{7}{c}{100} \\
        BERT config.& \multicolumn{7}{c}{12 layers, 768 hidden units, 12 heads} \\
        Batch size & & & & & & \\
        Learning rate  & & & & & & \\
        $L2$-reg weight & & & & & &  \\
        
        \bottomrule 
    \end{tabular}
    }
    \caption{Default hyper-parameters of our models. For the usage of $c$ and $w_\text{ctx}$, please refer to Algorithm~\ref{alg:pseudocode_st_extraction} and Algorithm~\ref{alg:pseudocode_aspair_building}.}
    \label{tab:parameters}
\end{table}

==> tables/pmi_seeds.tex <==
\newcolumntype{S}{>{\raggedright\arraybackslash}p{\linewidth}}

\begin{table}
    \centering
    \resizebox{\linewidth}{!}{%
    \begin{tabular}{S}
    \toprule
        \textsc{Positive words}  \\
         great, good, like, just, will, well, even, love, best, better, back, want, recommend, worth, easy, sound, right, excellent, nice, real, fun, sure, pretty, interesting, stars\\
        \midrule
        \textsc{Negative word} \\
        too, little, bad, game, down, long, hard, waste, disappointed, problem, try, poor, less, boring, worst, trying, wrong, least, although, problems, cheap \\
        \bottomrule
    \end{tabular}}
    \caption{Seed words $s^+$ and $s^-$ used for PMI-based sentiment term extraction}
    \label{tab:pmi_seeds}
\end{table}
